Can Stories Help LLMs Reason? Curating Information Space Through Narrative

Narratives are widely recognized as a powerful tool for structuring information and facilitating comprehension of complex ideas in various domains such as science communication. This paper investigates whether incorporating narrative elements can assist Large Language Models (LLMs) in solving complex problems more effectively. We propose a novel approach, Story of Thought (SoT), integrating narrative structures into prompting techniques for problem-solving. This approach involves constructing narratives around problem statements and creating a framework to identify and organize relevant information. Our experiments show that using various LLMs with SoT consistently surpasses using them with other techniques on physics, chemistry, math, and biology questions in both the GPQA and JEEBench datasets. The narrative-based information curation process in SoT enhances problem comprehension by contextualizing critical in-domain information and highlighting causal relationships within the problem space.

==> latex/02-related-work.tex <==
%%----------------------------------------------------
\section{Related Work}
\label{sec:relatedwork}
%%----------------------------------------------------

%%----------------------------------------------------
\paragraph{Narrative}
\label{subsec:Narrative}
%%----------------------------------------------------
\textit{Narrative}, as a noun, refers to a story or a description of a series of events~\footnote{\url{https://dictionary.cambridge.org/}}. In other words, it is a particular way of explaining or understanding events and plays a crucial role in human communication and cognition~\cite{hineline2018narrative}. The terms ``story'' and ``narrative'' are often used interchangeably. However, there is a subtle difference between them. A ``story'' is a narrative's content or substance, while a ``narrative'' is the structure or way the story is presented~\cite{abbott2020cambridge}.
Narrative plays a crucial role in various aspects of human communication and cognition. \citet{bruner1991narrative} argues that narrative is a fundamental mode of human thought, allowing individuals to organize and make sense of their experiences. However, there are also potential disadvantages to using narrative. One concern is that narratives can oversimplify complex issues or events, leading to a reductionist understanding~\cite{dahlstrom2012ethical}. Furthermore, an over-reliance on narrative structures may limit the exploration of alternative viewpoints or non-linear forms of information presentation~\cite{negrete2004learning}. It is essential to balance the benefits of narrative and the need for a nuanced understanding of the problem space~\cite{avraamidou2009role}.

%%----------------------------------------------------
\paragraph{Narrative and Human Cognition}
\label{subsec:Human Brain on Narrative}
%%----------------------------------------------------

Research into \textit{narrative transportation} examines how individuals become cognitively and emotionally absorbed in stories. This immersive experience enhances emotional responses and alters attitudes and beliefs by aligning the listener's brain with the storyteller's~\cite{oschatz2020long,bilandzic2020emotional}. Neuroimaging techniques such as functional Magnetic Resonance Imaging (fMRI), Positron Emission Tomography (PET), and Magnetoencephalography (MEG) show differences in identified active brain regions involved in narrative comprehension compared to factual processing~\cite{sanford2012mind, armstrong2020stories, aboud2019fairy, coopmans2022electrophysiological}. 
Furthermore, presenting information in narratives can enhance learning and memory, as well as promote engagement and motivation~\cite{willingham2004ask, rowe2010integrating, chen2023design}, which led to the development of narrative-based educational strategies~\cite{bower1969narrative, mawasi2020systematic, norris2005theoretical}. %These studies highlight how narratives significantly influence human cognition, emotion, and learning, revealing the complex neural interactions involved in narrative comprehension.

%%----------------------------------------------------
\paragraph{Role of Narrative in Solving Tasks}
\label{subsec:role-of-narrative}
%%----------------------------------------------------
In problem-solving, narratives can serve as a framework for organizing and presenting information relevant to the task~\cite{jonassen2002case, andrews2009storytelling}. Structuring the problem space as a narrative makes it easier to identify key elements, such as characters, goals, obstacles, and potential solutions~\cite{san2012getting}. Narratives can also help to break down complex problems into sub-problems, providing a step-by-step approach to problem-solving~\cite{szurmak2013tell}. For example, progressive disclosure, analogy, and analogical reasoning are powerful narrative techniques that facilitate problem-solving~\cite{salvucci2001integrating, gick1980analogical}. These techniques involve presenting information gradually in sub-problems, drawing comparisons and similarities between two seemingly disparate concepts, and using these similarities to generate insights or solutions~\cite{norris2005theoretical, holyoak1989computational}.

%%----------------------------------------------------
\paragraph{Narrative and LLM Prompting}
%%----------------------------------------------------
%\todo{Needs more details}
The intuitive approach to improving reasoning with LLMs is prompt engineering (see recent survey in \citet{qiao-etal-2023-reasoning}. %One of the most common prompting techniques is zero-shot learning, where the model is given a prompt without any examples or additional context. This approach relies solely on the model's inherent knowledge and understanding of language to generate appropriate responses.
Starting from CoT prompting~\citet{wei2022chain}, these techniques leverage LLMs' strong in-context learning ability, adding intermediate steps to generate a reasoning process before answering. 
While analogical reasoning can be a technique used in narrative generation, to our knowledge the narrative technique has never been fully explored as a coherent set of interconnected didactic approaches to improve the reasoning abilities of LLMs for problem-solving.

%Experiments suggest that CoT prompting helps LLMs improve their reasoning abilities. %\todo{\url{https://aclanthology.org/2023.acl-long.294.pdf}}


\if0
\begin{itemize}
  \item How do existing methods differ from one another and what are their 
  respective strenghts and weaknesses.
  \item How is this work challenging?
  \item Create context of the work.
  \item Create expectation of what the contribution of paper should be.
\end{itemize}

Narrative is used in various domains, including literature and storytelling, everyday communication, politics, games, and interactive media. Narrative is the primary means of conveying characters, plot, and themes in literature and storytelling. Everyday communication often involves sharing personal experiences and anecdotes, which are mini-narratives. In politics, narratives frame issues, persuade audiences, and shape public opinion. Political narratives can be powerful tools for mobilizing support or creating a shared identity. Games and interactive media increasingly employ narrative elements to create immersive experiences and engage users emotionally. The use of narrative in these contexts can range from simple backstories to complex branching storylines that respond to user choices.

\todo{LF: Maybe more something like "impact of narrative on human cognitive processes"?}

Analogy and analogical reasoning are powerful narrative techniques that can facilitate problem-solving. Analogies involve drawing comparisons between two seemingly disparate concepts or situations, highlighting their similarities and using these similarities to generate insights or solutions\cite{gentner1997structure}. By presenting a problem in the context of a familiar narrative or scenario, analogies can help individuals to better understand the problem and apply existing knowledge to generate novel solutions\cite{gick1980analogical}.

\todo{LF: Lots of stuff is needed here for this paper, maybe we even need two sections - the related work reviewing and defining the narrative term for our paper purpose can even go to Methodology or so}






\fi

==> latex/reviews.tex <==
Paper Summary:
The author propose a new variant of CoT (chain-of-thought), story-of-thought (SoT), to approach complex problems/tasks. Specifically, for each question, SoT prompts an LLM to identify important elements and knowledge concerning the given question, then generate a narrative conditioned on the intermediate information, and finally produce an answer based on the narrative. The author performs evaluation on GPQA and validate the effectiveness of this method.
Summary Of Strengths:
The idea of generative a story/narrative to construct the rationale space is novel and interesting. The proposed method -- Story of Thought -- is easy to understand.
Empirical results show that this prompting method is compatible with various underlying models (i.e., improvements over zero-shot baselines), except for Microsoft Phi-3 models.
Interesting analyses on narrative devices/elements (section 5.3 & 5.4). This provides a direct assessment of how useful each narrative technique is, and how LLMs are capable to to utilize each narrative technique in crafting a story.
Summary Of Weaknesses:
Related work on Chain-of-Y or X-of-Thought is needed considering the proposed method is a variant of CoT. More importantly, comparisons against existing CoT variants (e.g., tree-of-thought, graph-of-thought, program-of-thought) should be either quantitatively reported or qualitatively discussed.
Issues in experimental setting: 1) As LLMs can generate different responses when temperature is non-zero (line 311), how many runs are performed to obtain the accuracy? This is not reported, which needs more clarification; If it's just 1 run, then reported numbers and comparisons are not statistically reliable. 2) No few-shot experiments are conducted though it's explicitly stated that "showing superior performance to existing task-decomposition-based prompting techniques, such as zero-shot and few-shot chain of thought and analogical reasoning." (line78-81).
Issues in evaluation benchmarks: This study only evaluates the proposed method on only one dataset. This is not sufficient to conclude that this method can truly outperform select baselines. Also, which split of GPQA are you using? the main set or the diamond set?
Despite the fact that this is a intuitively simple prompting method, its computational process is unnecessarily complicated and the computational cost is increased. For each query/question, standard prompting and CoT can finish generating answers in one shot, while utilizing SoT requires prompting the LLM three times (see Figure 4). The value of this work will be certainly amplified if you could combine these three separate components into an end-of-end style.
Comments Suggestions And Typos:
It would be nice if you could provide which openAI endpoints you are using. For example, for GPT-3.5, there are various endpoints like 0613, and it's believed that performances of the same model are also different among different endpoints.
I personally suggest compressing this paper into a short paper considering that the actual content of this paper basically concludes on page 6. You may simply move the prompt templates to the appendix to save space.
How do you conduct the post-hoc processing? I doubt the solver always generates a response ending in "the correct answer is xxx".
Confidence: 4 = Quite sure. I tried to check the important points carefully. It's unlikely, though conceivable, that I missed something that should affect my ratings.
Soundness: 2 = Poor: Some of the main claims/arguments are not sufficiently supported. There are major technical/methodological problems.
Overall Assessment: 2 = Revisions Needed: This paper has some merit, but also significant flaws, and needs work before it would be of interest to the community.
Best Paper: No
Needs Ethics Review: No
Reproducibility: 3 = They could reproduce the results with some difficulty. The settings of parameters are underspecified or subjectively determined, and/or the training/evaluation data are not widely available.
Datasets: 1 = No usable datasets submitted.
Software: 4 = Useful: I would recommend the new software to other researchers or developers for their ongoing work.
Knowledge Of Or Educated Guess At Author Identity: No
Knowledge Of Paper: N/A, I do not know anything about the paper from outside sources
Knowledge Of Paper Source: N/A, I do not know anything about the paper from outside sources
Impact Of Knowledge Of Paper: N/A, I do not know anything about the paper from outside sources


Paper Summary:
The paper proposes a novel prompt design technique (SoT) based on the hypothesis that the narrative-based information curation process enhances understanding of LLM problems in complex reasoning tasks. The experimental results demonstrate SoT's consistent advantage over Chain of Thought (CoT) and analogical reasoning approaches in GPQA tasks.
Summary Of Strengths:
The authors proposed an interesting idea to generate narratives to provide a structured context for the original question to enhance the LLM’s understanding, reasoning, and problem-solving abilities. Experimental results show the utility of this prompt design.
Summary Of Weaknesses:
Defining "Complex Problem-Solving Tasks": Can you provide a more precise definition of "complex"? Does it encompass specific reasoning types?
Question Clarification: Are you using a single, pre-defined prompt for this step, or is there a method for generating the most effective prompt for each task?
Narrative Generation: Can you elaborate on the specific "techniques" used in narrative generation? How do each technique relate to criteria like "Branching"? Examples of prompts demonstrating these techniques would be helpful. Can the model be trained to automatically generate prompts based on the task, rather than relying on manual creation?
Phi-3 Model Performance: Table 1 shows no improvement for the Phi-3 model with SoT. Can you provide insights into why this might be the case?
Utilizing Different Models: Section 5.2 describes using a different model for narrative generation. If SoT is a pipeline, wouldn't a consistent model across all stages (problem classification, narrative generation, solving) be more efficient? Additionally, why are only results for Phi-3 shown?
Technique Consistency and Evaluation: Section 5.4 is unclear. Since LLMs are generative models, wouldn't the same SoT technique potentially generate different narratives each time? This raises questions about the experiment's validity. A more effective approach might be to identify consistently useful techniques and compare them to a control group with no SoT.
Dataset Information: The paper would benefit from details about the dataset used in the experiments, including type, size, and the number of samples analyzed.
Prompt level: Recent prompt designs are utilizing prompt taxonomies to categorize their design elements, facilitating fairer comparisons
Comments Suggestions And Typos:
No
Confidence: 4 = Quite sure. I tried to check the important points carefully. It's unlikely, though conceivable, that I missed something that should affect my ratings.
Soundness: 2.5
Overall Assessment: 2 = Revisions Needed: This paper has some merit, but also significant flaws, and needs work before it would be of interest to the community.
Best Paper: No
Limitations And Societal Impact:
Yes, they provide the limitations
Ethical Concerns:
No
Needs Ethics Review: No
Reproducibility: 3 = They could reproduce the results with some difficulty. The settings of parameters are underspecified or subjectively determined, and/or the training/evaluation data are not widely available.
Datasets: 3 = Potentially useful: Someone might find the new datasets useful for their work.
Software: 3 = Potentially useful: Someone might find the new software useful for their work.
Knowledge Of Or Educated Guess At Author Identity: No
Knowledge Of Paper: N/A, I do not know anything about the paper from outside sources
Knowledge Of Paper Source: N/A, I do not know anything about the paper from outside sources
Impact Of Knowledge Of Paper: N/A, I do not know anything about the paper from outside sources

Paper Summary:
This paper proposes a prompt method - Story of Thought (SoT), tailored for GPQA tasks. Based on a given question, SoT simply prompts LLM to first clarify the question, then generate corrsponding narrative, and finally answer the question with generated narrative. Results empirically demonstrates its effectiveness on GPQA tasks.
Summary Of Strengths:
The method is simple and easy to follow.
Results empirically demonstrates SoT's effectiveness on GPQA tasks.
Summary Of Weaknesses:
Could SoT be applied in more complex scenarios? For example, for more abstract questions like higher-level math problems, is it possible to generate narratives?
Inadequate evaluation. SoT is only tested on GPQA, and could it outperform baselines in other datasets?
More baselines needed. There are many ideas should be considered as baselines, such as Tree-of-thoughts, and Graph-of-thoughts.
Related works only focus on narratives and other prompt methods for reasoning enhancement (e.g., ToT, GoT) should be included.
Comments Suggestions And Typos:
The authors may provide an ipynb file in anonymous codebase for reviewers to play with.
Confidence: 5 = Positive that my evaluation is correct. I read the paper very carefully and am familiar with related work.
Soundness: 2 = Poor: Some of the main claims/arguments are not sufficiently supported. There are major technical/methodological problems.
Overall Assessment: 2 = Revisions Needed: This paper has some merit, but also significant flaws, and needs work before it would be of interest to the community.
Best Paper: No
Needs Ethics Review: No
Reproducibility: 4 = They could mostly reproduce the results, but there may be some variation because of sample variance or minor variations in their interpretation of the protocol or method.
Datasets: 1 = No usable datasets submitted.
Software: 1 = No usable software released.
Knowledge Of Or Educated Guess At Author Identity: No
Knowledge Of Paper: N/A, I do not know anything about the paper from outside sources
Knowledge Of Paper Source: N/A, I do not know anything about the paper from outside sources
Impact Of Knowledge Of Paper: N/A, I do not know anything about the paper from outside sources

